NNLander-VeriF: A Neural Network Formal Verification Framework for Vision-Based Autonomous Aircraft Landing

In this paper, we consider the problem of formally verifying a Neural Network (NN) based autonomous landing system. In such a system, a NN controller processes images from a camera to guide the aircraft while approaching the runway. A central challenge for the safety and liveness verification of vision-based closed-loop systems is the lack of mathematical models that captures the relation between the system states (e.g., position of the aircraft) and the images processed by the vision-based NN controller. Another challenge is the limited abilities of state-of-the-art NN model checkers. Such model checkers can reason only about simple input-output robustness properties of neural networks. This limitation creates a gap between the NN model checker abilities and the need to verify a closed-loop system while considering the aircraft dynamics, the perception components, and the NN controller. To this end, this paper presents NNLander-VeriF, a framework to verify vision-based NN controllers used for autonomous landing. NNLander-VeriF addresses the challenges above by exploiting geometric models of perspective cameras to obtain a mathematical model that captures the relation between the aircraft states and the inputs to the NN controller. By converting this model into a NN (with manually assigned weights) and composing it with the NN controller, one can capture the relation between aircraft states and control actions using one augmented NN. Such an augmented NN model leads to a natural encoding of the closed-loop verification into several NN robustness queries, which state-of-the-art NN model checkers can handle. Finally, we evaluate our framework to formally verify the properties of a trained NN and we show its efficiency.

==> SEC5-Algorithm/algorithm.tex <==
\section{ALGORITHM}


\textbf{Definition.} A control system $\Sigma$ is a quadruple $\Sigma = (R^n,U,\mathcal{U},f)$, where:

\begin{itemize}
\item  $R^n$ is the state space
\item $U \in R^m $ is the input set
\item $\mathcal{U}$ is a subset of all piecewise continuous functions of the time from intervals of the form $]a,b[ \in R$ to $U$ with $a < 0$ and $b>0$
\item $f:R^n \times U \rightarrow R^n$ is a continuous map satisfying the following Lipschitz assumption: for every compact set $Q \in R^n$, there exists a constant $L \in R^+$ such that for all $x,y \in Q$ and all $u \in U$, we have $||f(x,u)-f(y,u)|| \leq L ||x-y||$
\end{itemize}

A curve $\xi: \ ]a,b[ \rightarrow R^n$ is said to be a trajectory of $\Sigma$ if there exists $v \in \mathcal{U} $ satisfying $\dot \xi(t) = f(\xi(t), v(t))$ for almost all $t \in \ ]a,b[$. We also write $\xi_{xv}(\tau)$ to denote the point reached at time $\tau$  under the input $v$ from initial condition $x = \xi_{xv}(0)$.
\\

\textbf{Definition.} A control system $\Sigma$ is incrementally forward complete $\delta$-FC if it is forward complete and there exist continuous functions $\beta: R^+ \times R^+ \rightarrow R^+$ and $\gamma: R^+\times R^+ \rightarrow R^+$ such that for every $s \in R^+$, the functions $\beta(.,s)$ and $\gamma(.,s)$ belong to class $K_{\infty}$, the following condition is satisfied for all $t\in [0,\tau]$:

\begin{equation}
    ||\xi_{xv}(t) - \xi_{x'v'}(t)||\leq \beta(||x-x'||,t) + \gamma(||v-v'||_{\infty},t)
\end{equation}

Incremental forward completeness requires the distance between two arbitrary  trajectories to be bounded by the sum of two terms capturing the mismatch between the initial conditions and the mismatch between the input. We further restrict attention to sampled-data control systems, where input curves belong to $\mathcal{U_{\tau}}$ containing only constant curves of duration $\tau \in R^+$.
\\

\textbf{Definition:} Consider a control system $\Sigma = (R^n,U,u,f)$ and a smooth function $V:R^n \times R^n \rightarrow R_0^+$. Function $V$ is called a $\delta$-FC Lyapunov function for $\Epsilon$, if there exists $K_\infty$ functions $\underline \alpha, \overline \alpha, \rho$ and $k \in R$ such that:

\begin{enumerate}
    \item for any $x,x' \in R^n$:
    \begin{equation}
        \overline \alpha (||x-x'||)\leq V(x,x') \leq \overline \alpha(||x-x' ||)
    \end{equation}
    
    \item for any $x,x' \in R^n$ and for any $u,u' \in U$:
    \begin{equation}
        \frac{\partial V}{\partial x}f(x,u)+\frac{\partial V}{\partial x'}f(x',u') \leq kV(x,x') + \rho(||u-u'||)
    \end{equation}
    
\end{enumerate}

\textbf{Theorem (Zamani)} A control system $\Sigma=(R^n,U,u,f)$ is $\delta$-FC if it admits a $\delta-$FC Lyapunov function. Moreover the functions $\beta$ and $\gamma$ are given by:

\begin{equation}
    \beta(r,t)=\underline {a}^{-1}(2e^{kt}\overline{a}(r))
\end{equation}

\begin{equation}
    \gamma(r,t)=\underline{a}^{-1}(2\frac{e^{kt}-1}{k}\sigma(r))
\end{equation}

It has been shown [3] that symbolic models exist if the control systems satisfy an incremental forward completness assumption which is an incremental version of forward completeness. For every nonlinear control system satisfying the incremental forward completeness assumption, one can construct a symbolic model that is alternatingly approximately simulated by the control system and that approximately simulates the control system.
\\

Given a sampling time $\tau \in R^+$ and a control system $\Sigma = (R^n,U,\mathcal{U}_{\tau},f)$, consider the system $\Sigma_{\tau}=S_{\tau}(\Sigma)=(X_{\tau}, U_{\tau}, \rightarrow Y_{\tau}, H_{\tau})$. This system can be though of as the time discretization of the control system $\Sigma$. Indeed, a finite state run of $S_{\tau}(\Sigma)$ captures the state evolution of the control system $\Sigma$ at times $t=0,\tau,...,N\tau$. We consider a $\delta-FC$ control system $\Sigma =(R^n,U,\mathcal{U}_{\tau},f)$ and a quadruple $q=(\tau, \eta, \mu, \theta)$ of quantization parameters, where $\tau \in R^n$ is the sampling time, $\eta \in R^+$ is the state space quantization, $\mu \in R^+$ is the input set quantization, and $\theta \in R^+$ is a design parameter. Define the system:

\begin{equation}
    \Sigma_q=S_q(\Sigma)=(X_q, U_q, \rightarrow, Y_q, H_q)
\end{equation}

consisting of:
\\

\begin{itemize}
\item  $X_q = [R^n]_{\eta}$ 
\item $U_q = [U]_{\mu}$ 
\item $x_q \rightarrow x'_q$ if $||\xi_{x_qu_q}(\tau)-x'_q||\leq \beta(\theta,\tau)+\gamma(\mu,\tau)+\eta$
\item $Y_q = R^n$
\item $H_q = i : X_q \rightarrow Y_q$
\end{itemize}

The transition relation of $S_q(\Sigma)$ is well defined in the sense that for every $x_q \in X_q$ and every $u_q \in U_q$ there always exists $x'_q \in X_q$ such that $x_q \rightarrow x'_q$. This can be seen by noting that that by definition of $X_q$, for any $x \in R^n$ there always exists a state $x'_q \in X_q$ such that $||x-x'_q|| \leq \eta$. Hence, for $x=\xi_{x_qu_q}(\tau)$ there always exists a state $x'_q \in X_q$ satisfying $||\xi_{x_qu_q}(\tau) - x'_q || \leq \eta \leq \beta(\theta,\tau)+\gamma(\mu,\tau)+\eta$.
\\

\textbf{Theorem (Zamani)} Let $\Sigma=(R^n,U,\mathcal{U},f)$ be a $\delta-FC$ control system. For any desired precision $\epsilon \in R^+$, and any quadruple $q=(\tau, \eta, \mu, \theta)$ of quantization parameters satisfying $\mu \leq \bar \mu $ and $\eta \leq \epsilon \leq \theta$, we have:

\begin{equation}
    S_\tau(\Sigma) \preceq^{\epsilon}_S S_q(\Sigma)
\end{equation}

% % subsection main_algorithm (end)
% \setlength{\textfloatsep}{5pt}
% \IncMargin{0.5em}
% \begin{algorithm}[!t]

% \SetKwData{false}{False}
% \SetKwData{true}{True}
% \SetKwData{succArray}{succArray}
% \SetKwData{w}{W}
% \SetKwData{b}{b}
% \SetKwData{ver}{verified}


% \SetKwFunction{verifyTLLNN}{TraverseHyperplaneRegions}
% \SetKwFunction{isempty}{IsEmpty}

% \SetKwFunction{sat}{SATsolver}
% \SetKwFunction{maxx}{Maximize}
% \SetKwFunction{init}{init}
% \SetKwFunction{initbools}{createBooleanVariables}
% \SetKwFunction{append}{Append}
% \SetKwFunction{satq}{SAT?}
% \SetKwFunction{checkfeas}{CheckFeas}
% \SetKwFunction{truevars}{TrueVars}

% \SetKwData{i}{i}
% \SetKwData{IOta}{iota}
% \SetKwData{sol}{sol}

% \SetKwData{q_{center}}{q_{center}}

% \SetKwFunction{init}{Initialize}
% \SetKwFunction{solve}{Solve}
% \SetKwFunction{nom}{NominalFSM}
% \SetKwFunction{qcenter}{q_{centers}}
% \SetKwFunction{qtrans}{q_{transit}}
% \SetKwFunction{qce}{q_{CE}}
% \SetKwFunction{status}{status}
% \SetKwFunction{part}{Partition}
% \SetKwFunction{trans}{NomTransit}
% \SetKwFunction{FSM}{FsmBuilder}

% \SetKw{Break}{break}
% \SetKw{not}{not}
% \SetKw{In}{in}
% \SetKw{ret}{return}
% \SetKw{false}{False}

% \SetKwInOut{Input}{input}
% \SetKwInOut{Output}{output}

% %\SetKwRet{\Return}{return}
% \Input{
% \hspace{3pt}$f,g$ system dynamics \eqref{eq:system_dynamics} \\
% \hspace{3pt}$Y_\textsf{ws}$ workspace set \\
% \hspace{3pt}$NN$ controller to verify \\
% \hspace{3pt}$T$ Time horizon \\
% \hspace{3pt}$\tau$ sampling time \\
% \hspace{3pt}$\eta$ state space precision\\
% \hspace{3pt}$\phi$ safety property\\
% % \hspace{15pt}of $\mathcal{L}$ (poset base)
% }
% \Output{
% \hspace{3pt}\qtrans, \status
% }
% \BlankLine
% \SetKwProg{Fn}{function}{}{end}%
% \Fn{\nom{$f,g$,$Y_\textsf{ws}$,$\bar{NN}$,$T$,$\tau$,$\eta$,$\phi$}}{

%     \BlankLine

% 	\qcenter $\leftarrow$ \part($Y_\textsf{ws}$,$\eta$)
	
% 	\qtrans $\leftarrow$ \trans($q_{centers}$,$f,g$,$NN$,$T$,$\tau$)
	
% 	\status $\leftarrow$ \FSM($q_{transit}$,$T$,$\phi$)

% 	\BlankLine

% 	\eIf{\status==$SAT$}{
% 		\ret \qce 
		
% 	}{
% 		\ret \qtrans
% 	}
% }


% \caption{\texttt{NNLander-VeriF}.}
% \label{alg:repair_TLL}
% \end{algorithm}
% \DecMargin{0.5em}


